Low-Rank Adaptation of Deep Prior Neural Networks For Room Impulse Response Reconstruction

The Deep Prior framework has emerged as a powerful generative tool which can be used for reconstructing sound fields in an environment from few sparse pressure measurements. It employs a neural network that is trained solely on a limited set of available data and acts as an implicit prior which guides the solution of the underlying optimization problem. However, a significant limitation of the Deep Prior approach is its inability to generalize to new acoustic configurations, such as changes in the position of a sound source. As a consequence, the network must be retrained from scratch for every new setup, which is both computationally intensive and time-consuming. To address this, we investigate transfer learning in Deep Prior via Low-Rank Adaptation (LoRA), which enables efficient fine-tuning of a pre-trained neural network by introducing a low-rank decomposition of trainable parameters, thus allowing the network to adapt to new measurement sets with minimal computational overhead. We embed LoRA into a MultiResUNet-based Deep Prior model and compare its adaptation performance against full fine-tuning of all parameters as well as classical retraining, particularly in scenarios where only a limited number of microphones are used. The results indicate that fine-tuning, whether done completely or via LoRA, is especially advantageous when the source location is the sole changing parameter, preserving high physical fidelity, and highlighting the value of transfer learning for acoustics applications.

==> images/rir_image.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Micophone Position Analysis: non uniform grid of mics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{%
yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
},%
scaled y ticks=false}%
\begin{tikzpicture}%
% big figure 
\begin{axis}[%
            name=rirImg,
            width = 0.65\columnwidth,
            xlabel=$m$,
            ylabel=Time,
            y unit=\second,
            label style={font=\tiny},
            colorbar,
            point meta min=-1,
            point meta max=1,
            colorbar style={
                at={(1.02,1.0)},
                %title=$\mathrm{dB}$,
                % yticklabel style={
                %         /pgf/number format/precision=1,
                % },
                label style={font=\tiny},
                colormap/blackwhite,
                width=6pt
            },
            every tick label/.append style={font=\tiny},
            point meta= explicit, 
            % axis equal image, 
             % every tick label/.append style={font=\tiny},
            tick align=outside,
            % xtick = \empty,
            % ytick = \empty,
            title={\tiny$\mathbf{h}$},
            axis on top,
            colormap/blackwhite,
            xmax=32,
            xmin=1,
            ymax=0.03,
            ymin=0,
            y dir = reverse
        ]
        \addplot [matrix plot*,point meta=explicit,mesh/cols=32] file {images/data/rir_image.txt};
            % define coordinates at bottom left and top left of rectangle
        \coordinate (c1) at (axis cs:19.5,0);
        \coordinate (c2) at (axis cs:20.5,0.03);
        % draw a rectangle
        \draw (c1) rectangle (c2);
\end{axis}
% zoom figure 
\begin{axis}[
        name=zoomRIR,
        at={($(rirImg.south east)+(1cm,0.3cm)$)},
        title={\tiny${h}_{20}$},
        width=0.45\columnwidth,
        every tick label/.append style={font=\tiny},
        point meta min=-1,
        point meta max=1,
        point meta= explicit, 
        xmin = 0, 
        xmax= 0.03,
        xlabel=Time, 
        % ylabel=Amplitude, 
        label style={font=\tiny},
        x unit = \second,
        % ylabel near ticks, 
        xtick = \empty,
        ytick = \empty,
         ]
        \addplot[black] file {images/data/rir.txt};
\end{axis}  
	% draw dashed lines from rectangle in first axis to corners of second
    \draw [dashed] (c2) -- (zoomRIR.south east);
    \draw [dashed] (c1) -- (zoomRIR.north west);
\end{tikzpicture}

==> images/scheme.tex <==
\begin{tikzpicture}[
    conv/.style={rectangle, draw=black, minimum width=1.5cm, minimum height=1cm, fill=blue!10},
    lora/.style={rectangle, draw=red!80!black, dashed, minimum width=1.2cm, minimum height=0.5cm, fill=red!20},
    frozen/.style={rectangle, draw=gray, minimum width=1.5cm, minimum height=1cm, fill=gray!20},
    arrow/.style={-Stealth, thick},
    label/.style={font=\small}
]

% --- PRETRAINING ---
\node at (0,4.5) {\textbf{(a) Pretraining (Room A)}};

% Layers
\node[conv] (z1) at (0,3) {Noise $\mathbf{z}$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Micophone Position Analysis: non uniform grid of mics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{%
yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
},%
scaled y ticks=false}%
\begin{tikzpicture}%
% big figure 
\begin{axis}[%
            name=rirImg,
            width = 0.65\columnwidth,
            xlabel=$m$,
            ylabel=Time,
            y unit=\second,
            label style={font=\tiny},
            colorbar,
            point meta min=-1,
            point meta max=1,
            colorbar style={
                at={(1.02,1.0)},
                %title=$\mathrm{dB}$,
                % yticklabel style={
                %         /pgf/number format/precision=1,
                % },
                label style={font=\tiny},
                colormap/myviolet,
                width=6pt
            },
            every tick label/.append style={font=\tiny},
            point meta= explicit, 
            % axis equal image, 
             % every tick label/.append style={font=\tiny},
            tick align=outside,
            % xtick = \empty,
            % ytick = \empty,
            title={\tiny$\mathbf{H}$},
            axis on top,
            colormap/myviolet,
            xmax=32,
            xmin=1,
            ymax=0.03,
            ymin=0,
            y dir = reverse
        ]
        \addplot [matrix plot*,point meta=explicit,mesh/cols=32] file {./images/data/rir_image.txt};
            % define coordinates at bottom left and top left of rectangle
        \coordinate (c1) at (axis cs:19.5,0);
        \coordinate (c2) at (axis cs:20.5,0.03);
        % draw a rectangle
        \draw (c1) rectangle (c2);
\end{axis}
% zoom figure 
\begin{axis}[
        name=zoomRIR,
        at={($(rirImg.south east)+(1cm,0.3cm)$)},
        title={\tiny$\mathbf{h}_{20}$},
        width=0.45\columnwidth,
        every tick label/.append style={font=\tiny},
        point meta min=-1,
        point meta max=1,
        point meta= explicit, 
        xmin = 0, 
        xmax= 0.03,
        xlabel=Time, 
        % ylabel=Amplitude, 
        label style={font=\tiny},
        x unit = \second,
        % ylabel near ticks, 
        xtick = \empty,
        ytick = \empty,
         ]
        \addplot[blue] file {images/data/rir.txt};
\end{axis}  
	% draw dashed lines from rectangle in first axis to corners of second
    \draw [dashed] (c2) -- (zoomRIR.south east);
    \draw [dashed] (c1) -- (zoomRIR.north west);
\end{tikzpicture}\node[conv, right=1.8cm of z1] (enc1) {Encoder};
\node[conv, right=1.8cm of enc1] (bottleneck) {Bottleneck};
\node[conv, right=1.8cm of bottleneck] (dec1) {Decoder};
\node[conv, right=1.8cm of dec1] (out1) {$\hat{\mathbf{h}}$};

% Arrows
\draw[arrow] (z1) -- (enc1);
\draw[arrow] (enc1) -- (bottleneck);
\draw[arrow] (bottleneck) -- (dec1);
\draw[arrow] (dec1) -- (out1);

% --- LORA ADAPTATION ---
\node at (0,0.5) {\textbf{(b) LoRA Adaptation (Room B)}};

% Frozen layers + Lora
\node[frozen] (z2) at (0,-1) {Noise $\mathbf{z}$};
\node[frozen, right=1.8cm of z2] (enc2) {Encoder};
\node[frozen, right=1.8cm of enc2] (bottleneck2) {Bottleneck};
\node[frozen, right=1.8cm of bottleneck2] (dec2) {Decoder};
\node[frozen, right=1.8cm of dec2] (out2) {$\hat{\mathbf{h}}'$};

% LoRA blocks
\node[lora, below=0.1cm of enc2] (lora1) {LoRA};
\node[lora, below=0.1cm of bottleneck2] (lora2) {LoRA};
\node[lora, below=0.1cm of dec2] (lora3) {LoRA};

% Arrows
\draw[arrow] (z2) -- (enc2);
\draw[arrow] (enc2) -- (bottleneck2);
\draw[arrow] (bottleneck2) -- (dec2);
\draw[arrow] (dec2) -- (out2);

% LoRA connections
\draw[arrow, red, dashed] (lora1.north) -- (enc2.south);
\draw[arrow, red, dashed] (lora2.north) -- (bottleneck2.south);
\draw[arrow, red, dashed] (lora3.north) -- (dec2.south);

% Labels
\node[label, below=0.8cm of out2] (label1) {Frozen weights $\mathbf{W}$};
\node[label, below=0.2cm of label1] {Trainable LoRA $\Delta \mathbf{W} = \alpha \mathbf{B} * \mathbf{A}$};

\end{tikzpicture}
